CFNet: Learning Correlation Functions for One-Stage Panoptic Segmentation

Recently, there is growing attention on one-stage panoptic segmentation methods which aim to segment instances and stuff jointly within a fully convolutional pipeline efficiently. However, most of the existing works directly feed the backbone features to various segmentation heads ignoring the demands for semantic and instance segmentation are different: The former needs semantic-level discriminative features, while the latter requires features to be distinguishable across instances. To alleviate this, we propose to first predict semantic-level and instance-level correlations among different locations that are utilized to enhance the backbone features, and then feed the improved discriminative features into the corresponding segmentation heads, respectively. Specifically, we organize the correlations between a given location and all locations as a continuous sequence and predict it as a whole. Considering that such a sequence can be extremely complicated, we adopt Discrete Fourier Transform (DFT), a tool that can approximate an arbitrary sequence parameterized by amplitudes and phrases. For different tasks, we generate these parameters from the backbone features in a fully convolutional way which is optimized implicitly by corresponding tasks. As a result, these accurate and consistent correlations contribute to producing plausible discriminative features which meet the requirements of the complicated panoptic segmentation task. To verify the effectiveness of our methods, we conduct experiments on several challenging panoptic segmentation datasets and achieve state-of-the-art performance on MS COCO with $45.1$\% PQ and ADE20k with $32.6$\% PQ.

==> sections/intro_xili.tex <==
\section{Introduction}
Panoptic segmentation~\cite{kirillov2019panoptic1}, a fundamental and challenging problem in scene parsing, is to carry out instance segmentation for foreground things and semantic segmentation for background stuff.
%As a fundamental and challenging problem in scene parsing, panoptic segmentation~\cite{kirillov2019panoptic1} has gained considerable attention in recent years. It aims to carry out instance segmentation for foreground things and semantic segmentation for background stuff.
%Therefore, panoptic segmentation is a position-sensitive hybrid task that requires adaptive learning strategies w.r.t. different types of regions (foreground or background). In this paper, we focus on building effective positional encoding models for dynamically capturing the pixel-adaptive contextual interactions with different patterns for foreground and background.
\begin{figure}[tb]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/intro_ills_1_v4}
	\caption{
%        (a) demonstrates the different needs of positional encodings for semantic and instance segmentations. We indicate pixel affinity with the similarity of colors.
%        (b)(c) illustrates that static positional encodings are not robust against scene changes.
%        In (b) and (c), we take coordinates as static positional encodings and visualize them via gradient-style colors.
%        The distinction between instances is indicated by the contrast of their average colors, which are shown in the squares linked to them.
%        As we can see, (b) presents cases that positional encodings are helpful for the tasks, while (c) presents cases in which static positional encodings are inadequate.
%        Specifically in (c), \textcircled{3} is considered closer to \textcircled{4} rather than its kin \textcircled{1} in semantic segmentation, and \textcircled{2} \textcircled{3} are indistinguishable even though they are spatially distant in instance segmentation.
		(a) demonstrates the different needs of positional encodings for semantic segmentation~(SS) and instance segmentation~(IS).
		Pixel affinity is indicated with the similarity of colors.
		In (b)(c), we take coordinates as positional encodings and map them to gradient-style colors. The average color of each instance is indicated by a cursor upon a color bar. The closer two cursors get, the more similar their corresponding encodings are.
		%For clear comparison, we quantize the colors of the objects and project them to a one-dimensional line under the images.
		%Each colored bar represents an object, and nearby bars indicate more relevant objects.
		(b) shows situations where static encodings can be helpful. In SS, the encodings suggest the helpful cue that \textcircled{2} is more relevant to \textcircled{1} than \textcircled{4}. In IS, the encodings of \textcircled{1}\textcircled{2}\textcircled{3} are distant, which helps distinguish them.
		(c) gives cases to show that static encodings are not robust to scene changes. In SS, \textcircled{3} is considered as more relevant to \textcircled{4} (another category) rather than \textcircled{1}(same category). In IS, the encodings of spatially distant \textcircled{2} and \textcircled{3} are indistinguishable.
		\label{fig:illustration}
	}
\end{figure}


%In the literature, a number of segmentation approaches resort to different kinds of positional information
%for enhancing the feature representation capability.
Recently, there is a growing recognition that positional information is helpful for scene understanding.
For example, semantic segmentation tasks build attention mechanisms in conjunction with positional encodings~\cite{wang2020axial, wang2018location} to model the prior knowledge that pixels close to each other are likely to be correlated.
In instance-aware tasks~(\eg object detection and instance segmentation), the spatial constraints on pixel features are explicitly enforced~\cite{liu2018intriguing, wang2020solo}, which ensures that the feature representations for spatially distant pixels ought to differ mutually.
However, there is a dilemma that the above two tasks have different positional encoding demands (sometimes even conflicting).
As illustrated in Fig.~\ref{fig:illustration}(a), semantic segmentation aims to diminish the difference among instances of the same class, while instance segmentation tries to maintain their distinction.
%Therefore, it is indispensable to provide different forms of positional encodings for different segmentation tasks.
Therefore, it is indispensable to provide different positional encodings for different segmentation tasks.
It is noted that existing panoptic segmentation approaches either partially satisfy~\cite{chen2020panonet, gao2020learning, wang2020axial} or ignore~\cite{chen2019pdeeplab, wang2020pixel} the different needs of positional information.
Besides, their positional encoding patterns are usually static~(\ie irrelevant to input scenes), such as fixed functions of coordinates~\cite{carion2020end, liu2018intriguing} or learned embeddings~\cite{ramachandran2019stand, wang2020axial}, resulting in the low flexibility of handling enormous and various scenes.
As illustrated in Fig.~\ref{fig:illustration}(b) and (c), static positional encodings provide rigid correlations among pixels regardless of scene changes, which are not always intuitive.


Motivated by the above observations, we propose a learnable dynamic positional encoding mechanism, which generates adaptive positional encodings for semantic and instance segmentation tasks.
The proposed mechanism is able to capture task-specific, scene-adaptive positional correlations among pixels so that the intra-class distance reduction in semantic segmentation and inter-instance distinction increase in instance segmentation can be well balanced.
Specifically, we model the positional correlation between a pixel and the other pixels as a learnable function of positions formed by two parameterized orthogonal periodic signals to dynamically reflect the actual positional information in the semantic or instance-aware context.
In semantic segmentation, the correlation among pixels corresponds to the affinity information, which is used for feature propagation to reinforce the connections between correlated pixels.
In instance segmentation, we select a fixed number of reference points, and take the correlation maps between each pixel and these reference points as positional embeddings, which ensures that pixels belong to different instances are distinctive.
The above task-specific signal parameters are learned in a single-stage pipeline without direct supervision.

Our method is advantageous in the following aspects.
Firstly, we provide different forms of positional encodings for instance and semantic segmentations so that the aforementioned demand conflict between tasks is avoided.
Besides, our method dynamically models positional correlation among pixels while taking scene content into account.
At last, our method can easily be parallelized, and thus is computationally efficient~(with an extra $8ms$ overhead).

In summary, the contributions of our work are as follows:
\begin{itemize}
	\item We propose a dynamic, fast, and label-free way to model positional information from the scene.
	\item We design two forms of positional encodings that are suitable for semantic segmentation and instance segmentation, respectively.
	\item We achieve a SOTA single-stage panoptic segmentation network with 85ms runtime and 42.3\% PQ.
\end{itemize}







